The chiral phase transition from strong to weak coupling

The order of the chiral phase transition of lattice QCD with unimproved staggered fermions is known to depend on the number of quark flavours, their masses and the lattice spacing. Previous studies in the literature for $N_f \in \{ 3,4 \}$ show first-order transitions, which weaken with decreasing lattice spacing. Here we investigate what happens when lattices are made coarser to establish contact to the strong coupling region. For $N_f \in \{4,8 \}$ we find a drastic weakening of the transition when going from $N_{\tau}=4$ to $N_{\tau}=2$, which is consistent with a second-order chiral transition reported in the literature for $N_f=4$ in the strong coupling limit. This implies a non-monotonic behaviour of the critical quark or pseudo-scalar meson mass, which separates first-order transitions from crossover behaviour, as a function of lattice spacing.

==> tikzlibraryspyall.code.tex <==
% Spy all styles

\tikzset{
  spy all using outlines/.style={
    spy picture={
      every spy all on node/.style={very thin,draw},
      every spy all in node/.style={thick,draw},
      #1
    }
  },
  spy all using overlays/.style={
    spy picture={
      every spy all on node/.style={fill,fill opacity=0.2,text opacity=1},
      every spy all in node/.style={fill,fill opacity=0.2,text opacity=1},
      #1
    }
  },
  connect spies/.style={
    spy connection path={\draw[thin] (tikzspyonnode) -- (tikzspyinnode);}
  }
}

%\newbox\tikz@lib@spybox

\let\tikz@lib@spyall@collection=\pgfutil@empty%

\tikzset{spy picture/.style={
    size/.style={minimum size=##1},
    height/.style={minimum height=##1},
    width/.style={minimum width=##1},
    execute at begin picture={%
      \let\tikz@lib@spyall@save=\tikz@lib@spyall@collection%
      \let\spyall=\tikz@lib@spyall@parse%
      \tikz@insert@spy@layer
      \pgfonlayer{spy}%
    },
    execute at end picture={%
      \endpgfonlayer
      {%
        \tikz@lib@spyall@collection%
      }%
      \global\let\tikz@lib@spyall@collection=\tikz@lib@spyall@save%
    },%
    tikz@lib@spyall@style/.style={#1},
    tikz@lib@reset@gs
  },
  lens/.store in=\tikz@lib@spy@lens,
  lens=,
  magnification/.style={lens={scale=#1}},
  spy connection path/.store in=\tikz@lib@spy@path,
  spy connection path=
}

\tikzset{
  tikz@lib@reset@gs/.style={black,thin,solid,opaque,line cap=butt,line join=miter}
}

\def\tikz@lib@spyall@parse{%
  \pgfutil@ifnextchar[{\tikz@lib@spyall@parse@opt}{\tikz@lib@spyall@parse@opt[]}%]
}
\def\tikz@lib@spyall@parse@opt[#1]{
  \pgfutil@ifnextchar x{\tikz@lib@spyall@parse@opta[#1]}{\tikz@lib@spyall@parse@opta[#1]}%]
}
\def\tikz@lib@spyall@parse@opta[#1]on#2in node#3;{%
  \pgfutil@g@addto@macro\tikz@lib@spyall@collection{\tikz@lib@spyall@do{#1}{#2}{#3}}%
}

\def\tikz@lib@spyall@do#1#2#3{%
  \scope[tikz@lib@spyall@style,#1]
    \node [alias=tikzspyonnode,inner sep=0pt,outer sep=0pt,every spy all on node/.try,
    /utils/exec={
      {%
        \let\tikz@transform=\relax
        \pgftransformreset%
        \expandafter\tikzset\expandafter{\tikz@lib@spy@lens}
        \pgftransforminvert%
        \pgfgettransformentries\a\b\c\d\e\f%
        \global\let\pgf@lib@svg@a=\a%
        \global\let\pgf@lib@svg@b=\b%
        \global\let\pgf@lib@svg@c=\c%
        \global\let\pgf@lib@svg@d=\d%
      }%
      \tikz@addtransform{%
        \tikz@scan@one@point\pgftransformshift#2%
        \pgftransformcm{\pgf@lib@svg@a}{\pgf@lib@svg@b}{\pgf@lib@svg@c}{\pgf@lib@svg@d}{\pgfpointorigin}%
      }
    }]{};
    \node [alias=tikzspyinnode,inner sep=0pt,outer sep=0pt,at={#2},every spy all in node/.try,
    path picture={\node[anchor=center,tikz@lib@reset@gs]{\nullfont%
        \pgfpicture\relax\pgfsetbaseline{default}\pgfsettrimleft{default}\pgfsettrimright{default}%
        \pgftransformreset%
        \let\tikz@transform=\relax%
        \expandafter\tikzset\expandafter{\tikz@lib@spy@lens}%
        \pgflowlevelsynccm%
        \tikz@scan@one@point\tikz@lib@spyall@shift#2%
        \pgflowlevelsynccm%
        \pgf@dosavedlayers
        \endpgfpicture};}]#3{};
    \tikz@lib@spy@path
  \endscope
}

\def\tikz@lib@spyall@shift#1{%
  \pgf@process{#1}%
  \pgf@x=-\pgf@x%
  \pgf@y=-\pgf@y%
  \pgftransformshift{}%
}

\pgfdeclarelayer{spy}


\def\tikz@insert@spy@layer{%
    \expandafter\tikz@insert@spy@@layer\pgf@layerlist\relax
}
\def\tikz@insert@spy@@layer#1main#2\relax{%
    \def\pgf@layerlist{#1spy#2,main}%
}


\def\pgf@dosavedlayers{%
  \expandafter\pgf@dosavedlayer\pgf@layerlist,,\relax%
}
\def\pgf@dosavedlayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \copy\pgf@layerbox@main
  \else%
    \expandafter\copy\csname pgf@layerboxsaved@#1\endcsname
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavedlayer#2,\relax%
  \fi%
}
\newbox\pgf@layerboxsaved@main
\def\pgf@dosavelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \setbox\pgf@layerboxsaved@main=\box\pgf@layerbox@main
  \else%
    \setbox\csname pgf@layerboxsaved@#1\endcsname=\box\csname pgf@layerbox@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavelayer#2,\relax%
  \fi%
}


\endinput
